Local density dependent potential for compressible mesoparticles

We focus on finding a coarse grained description able to reproduce the thermodynamic behavior of a molecular system by using mesoparticles representing several molecules. Interactions between mesoparticles are modelled by an interparticle potential, and an additional internal equation of state is used to account for the thermic contribution of coarse grained internal degrees of freedom. Moreover, as strong non-equilibrium situations over a wide range of pressure and density are targeted, the internal compressibility of these mesoparticles has to be considered. This is done by introducing a dependence of the potential on the local environment of the mesoparticles, either by defining a spherical local density or by means of a Voronoi tessellation. As an example, a local density dependent potential is fitted to reproduce the Hugoniot curve of a model of nitromethane, where each mesoparticle represents one thousand molecules.

==> Illustrations/dv_correlation/readme <==
correlation : Correlation~\eqref{def_correl} between the Voronoi and local densities with respect to the local density cut-off radius $r_{\rm cut}$.

joint-dist : Joint distribution of the Voronoi and spherical densities at $r_{\rm cut} = 1.2 \, \sigma$ (red) and $r_{\rm cut} = 2.5 \, \sigma$ (blue).

==> Illustrations/dv_hist/readme <==
dst_hist : Distribution of the spherical ($r_{\rm cut} = 2.5\sigma$) and Voronoi densities at $\rho = 1650$~kg.m$^{-3}$

==> Illustrations/hugoniot/readme <==
hug_nm-s1 : Hugoniot curve for nitromethane: reference curve~\cite{desbiens_2009}
hug_nm2 : Hugoniot curve for nitromethane: reference curve~\cite{desbiens_2009} and results for density-dependent potentials with $p=0$ and $p=2$.

hug_pred : Hugoniot curve for nitromethane: Predicted values of the pressure outside the optimization range of the parameters.

==> Illustrations/opt_r0-global/readme <==
r0_global : Optimal $\lambda_0$ for the reference states with respect to the mean Voronoi volume $V_s = \frac{m_{\rm sys}}{\rho_{s}}$
